GLIP: Graph and LLM Joint Pretraining for Graph-Level Tasks

Graphs are widely used to model relational systems, with applications in domains such as social networks, finance, and biomedicine. Graph neural networks (GNNs) have become a mainstream approach for learning graph representations. With the rise of large language models (LLMs), recent studies have attempted to combine GNNs with LLMs. However, most existing works concentrate on node-level and edge-level tasks, while graph-level tasks, which require capturing more complex structural and feature information, remain relatively underexplored. Moreover, graph pretraining is a widely adopted strategy to alleviate the challenge of label scarcity. Most existing approaches are designed solely for GNNs such as GraphCL, leaving LLMs uninvolved in the process. To address these limitations, we propose GLIP, a Graph-LLM JoInt Pretraining framework for graph-level tasks. GLIP first performs graph augmentation to construct positive and negative pairs and introduces a multi-token selection strategy to identify patches informative in both structure and features. It further leverages a diffusion-based projector to enrich them with contextual information, enabling GLIP to capture signals from both global and local perspectives. Finally, GLIP employs a joint objective that integrates the LLM's semantic judgments with a contrastive alignment loss, ensuring consistent supervision at both the semantic and structural levels. After pretraining, GLIP is fine-tuned with limited labeled data for downstream tasks, and extensive experiments show that it outperforms state-of-the-art methods on graph-level classification and reasoning tasks. Our source code is publicly available at https://anonymous.4open.science/r/GLIP.

==> fg.tex <==
\usepackage{pgfplots}
\usepackage{graphicx}
\usepackage{xcolor}
\pgfplotsset{compat=1.18}

% 定义配色方案（取自你提供的图片）
\definecolor{cream}{RGB}{244,241,222}
\definecolor{coral}{RGB}{223,122,94}
\definecolor{navy}{RGB}{60,64,91}
\definecolor{mint}{RGB}{130,178,154}
\definecolor{sand}{RGB}{242,204,142}

\begin{figure}[htbp!]
    \centering
    \begin{tikzpicture}
    \begin{axis}[
        ybar,
        bar width=6pt,
        width=0.95\textwidth,
        height=0.48\textwidth,
        ylabel={Accuracy (\%)},
        symbolic x coords={PROTEINS, REDDIT, E-COM},
        xtick=data,
        ymin=50, ymax=90,
        ymajorgrids=true,
        grid style=dashed,
        legend style={
            at={(0.5,1.05)},
            anchor=south,
            legend columns=-1,
            column sep=6pt,
            font=\small
        },
        tick label style={font=\small},
        label style={font=\small},
        bar shift auto
    ]

    % ===== 数据部分（你后面可自行替换） =====
    % GLIP
    \addplot[fill=coral] coordinates {
        (PROTEINS,68.4) (REDDIT,87.2) (E-COM,86.3)
    };
    % w/o Pretrain
    \addplot[fill=navy] coordinates {
        (PROTEINS,64.1) (REDDIT,83.6) (E-COM,82.0)
    };
    % w/o PatchSelection
    \addplot[fill=mint] coordinates {
        (PROTEINS,66.2) (REDDIT,84.0) (E-COM,83.1)
    };
    % w/o Diffusion
    \addplot[fill=sand] coordinates {
        (PROTEINS,65.0) (REDDIT,85.1) (E-COM,84.5)
    };
    % w/ Random PatchSel
    \addplot[fill=cream, draw=gray!50] coordinates {
        (PROTEINS,66.7) (REDDIT,85.5) (E-COM,84.0)
    };

    \legend{GLIP, w/o Pretrain, w/o PatchSel, w/o Diffusion, w/ Random PatchSel}
    \end{axis}
    \end{tikzpicture}
    \caption{\textbf{Ablation study on three datasets.}
    Performance comparison of GLIP and its variants on PROTEINS, REDDIT, and E-COM datasets.}
    \label{fig:ablation}
\end{figure}

